A New Dataset for Natural Language Inference from Code-mixed Conversations

Natural Language Inference (NLI) is the task of inferring the logical relationship, typically entailment or contradiction, between a premise and hypothesis. Code-mixing is the use of more than one language in the same conversation or utterance, and is prevalent in multilingual communities all over the world. In this paper, we present the first dataset for code-mixed NLI, in which both the premises and hypotheses are in code-mixed Hindi-English. We use data from Hindi movies (Bollywood) as premises, and crowd-source hypotheses from Hindi-English bilinguals. We conduct a pilot annotation study and describe the final annotation protocol based on observations from the pilot. Currently, the data collected consists of 400 premises in the form of code-mixed conversation snippets and 2240 code-mixed hypotheses. We conduct an extensive analysis to infer the linguistic phenomena commonly observed in the dataset obtained. We evaluate the dataset using a standard mBERT-based pipeline for NLI and report results.

==> intro.tex <==
\section{Introduction}
Natural Language Inferencing (NLI) is one of the fundamental NLP tasks, not only because it has several practical applications, but also because it tests the language understanding abilities of the machines beyond pattern recognition. NLI tasks usually involve inferring the logical relationship, such as entailment or contradiction, between a pair of sentences. In some cases, instead of a sentence, a document, paragraph or a dialogue snippet might be provided as the {\em premise}; the task then is to infer whether a given {\em hypothesis} sentence is entailed (or implied) by the premise. There are several monolingual NLI datasets available, most notably the GLUE and SuperGLUE. There are also multilingual and crosslingual NLI datasets, such as XNLI. These datasets have successfully spurred and facilitated research in this area. \\

In this paper, we introduce, for the first time, a new NLI dataset for {\em code-mixing}. Code-mixing or code-switching refers to use of the more than one language in a single conversation or utterance. It is a prevalent phenomenon in almost all multilingual societies. Monolingual as well as multilingual NLP systems typically fail to handle code-mixed inputs. Therefore, recently, code-mixing has attained a considerable attention from the speech and NLP communities. Consequently, there have been several shared tasks on language labeling, POS-tagging and sentiment analysis of code-mixed text; several datasets exist for these as well as other speech and language processing tasks such speech recognition, parsing and question answering. However, as far as we know, there exists no code-mixed dataset for any NLI task.  \\

3 reasons for code-mixed NLI dataset: On the other hand, code-mixed NLI is an important end-application for chat bots because CM happens in chat - Alexa, Cortana etc. Also, it is not clear whether zeroshot learning can solve code-mixed NLI. NLI will tell us whether the machines truly understand CM. \\




Approach and dataset short summary \\

Organization


